CLAMP-ViT: Contrastive Data-Free Learning for Adaptive Post-Training Quantization of ViTs

We present CLAMP-ViT, a data-free post-training quantization method for vision transformers (ViTs). We identify the limitations of recent techniques, notably their inability to leverage meaningful inter-patch relationships, leading to the generation of simplistic and semantically vague data, impacting quantization accuracy. CLAMP-ViT employs a two-stage approach, cyclically adapting between data generation and model quantization. Specifically, we incorporate a patch-level contrastive learning scheme to generate richer, semantically meaningful data. Furthermore, we leverage contrastive learning in layer-wise evolutionary search for fixed- and mixed-precision quantization to identify optimal quantization parameters while mitigating the effects of a non-smooth loss landscape. Extensive evaluations across various vision tasks demonstrate the superiority of CLAMP-ViT, with performance improvements of up to 3% in top-1 accuracy for classification, 0.6 mAP for object detection, and 1.5 mIoU for segmentation at similar or better compression ratio over existing alternatives. Code is available at https://github.com/georgia-tech-synergy-lab/CLAMP-ViT.git

==> tables/joint_tables.tex <==
\begin{table}[!t]
    \centering % Center the entire table set
    \begin{minipage}[t]{0.48\linewidth}
        \centering
        \caption{List of parameters in CLAMP-ViT framework and their empirically determined values.}
        \label{tab:parameters}
        \scriptsize
        \begin{tabular}{ccc}
            \Xhline{2\arrayrulewidth}
            Parameter & Description & Value \\
            \Xhline{2\arrayrulewidth}
            $G$ & Generation Iterations & 500 \\
            $\mathcal{N}$ & Neighborhood Size & $3 \times 3$ \\
            $n$ & \# Positive Patches & 4 \\
            $\mathcal{P}$ & Passes & 10 \\
            $\mathcal{C}$ & Cycles & 6 \\
            $\mathcal{K}$ & \# Initial Candidates & 15 \\
            $\mathcal{B}$ & Batch Size & 32 \\
            $b$ & Bitwidth & [2,8] \\
            \Xhline{2\arrayrulewidth}
        \end{tabular}
        \vspace{-5mm}
    \end{minipage}\hfill % Use \hfill to push the second minipage to the right
    \begin{minipage}[t]{0.48\linewidth}
        \centering
        \caption{Impact on final quantization accuracy of different loss functions for guiding synthetic data generation. Multiple \cmark per row indicates linear combination.}
        \label{tab:loss_func}
        \scriptsize
        \begin{tabular}{ccccc}
            \Xhline{2\arrayrulewidth}
            $\mathcal{L}_{PSE}$ & $\mathcal{L}_{C}$ & $\mathcal{L}_{O}$ & W/A & Top-1 Accuracy  \\
            \Xhline{2\arrayrulewidth}
             - & - & - & 32/32 & 79.85 \\ \cline{1-5}
             \cmark & \xmark & \xmark & 4/8 & 74.18 \\
             \xmark & \xmark & \cmark & 4/8 & 33.93 \\
             \cmark & \xmark & \cmark & 4/8 & 76.47 \\
             \xmark & \cmark & \xmark & 4/8 & 76.59 \\ 
             \xmark & \cmark & \cmark & 4/8 & 77.03 \\
            \Xhline{2\arrayrulewidth}
        \end{tabular}
        \vspace{-5mm}
    \end{minipage}
\end{table}
